Towards Probing Speech-Specific Risks in Large Multimodal Models: A Taxonomy, Benchmark, and Insights

Large Multimodal Models (LMMs) have achieved great success recently, demonstrating a strong capability to understand multimodal information and to interact with human users. Despite the progress made, the challenge of detecting high-risk interactions in multimodal settings, and in particular in speech modality, remains largely unexplored. Conventional research on risk for speech modality primarily emphasises the content (e.g., what is captured as transcription). However, in speech-based interactions, paralinguistic cues in audio can significantly alter the intended meaning behind utterances. In this work, we propose a speech-specific risk taxonomy, covering 8 risk categories under hostility (malicious sarcasm and threats), malicious imitation (age, gender, ethnicity), and stereotypical biases (age, gender, ethnicity). Based on the taxonomy, we create a small-scale dataset for evaluating current LMMs capability in detecting these categories of risk. We observe even the latest models remain ineffective to detect various paralinguistic-specific risks in speech (e.g., Gemini 1.5 Pro is performing only slightly above random baseline). Warning: this paper contains biased and offensive examples.

==> figure_table/level2-small.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{9pt} %2.5pt
\centering
\scalebox{0.5}{ %0.6
\begin{tabular}{llcccccc}
\toprule
% &&\multicolumn{7}{c}{\bf Tasks}\\
% \cmidrule(lr){3-9}
%  Tr.&Model& SF  & SD  & QbE & KS & IC & PR$^*$ &ASR$^*$ \\
% &&\multicolumn{14}{c}{\bf Tasks}\\
 & & \multicolumn{2}{c}{Gender}  & \multicolumn{2}{c}{Age}  &  \multicolumn{2}{c}{Ethnicity}  \\
 \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 Model&Prompt& Acc   &F1& Acc   &F1  & Acc   &F1\\
 \midrule 
  &\multicolumn{3}{c}{\textbf{Gemini-1.5-Pro}}\\
  
 \multirow{2}{*}{Qwen-Audio-Chat-7B}
 &\text{Avg. Y/N (Level-1)}&51.94&39.64&51.00&43.81&49.44&33.79\\
 &\text{Avg. Y/N (Level-2)}&\textbf{54.41}&\textbf{46.35}&50.80&\textbf{44.42}&\textbf{50.14}&\textbf{34.12}\\

 
\midrule
\multirow{2}{*}{SALMONN-7B} 
&\text{Avg. Y/N (Level-1)}&51.94&39.56&49.53&33.35&50.28&34.17\\
 &\text{Avg. Y/N (Level-2)}&\textbf{54.73}&\textbf{42.80}&49.40&33.07&50.00&33.33\\

 
\midrule
\multirow{2}{*}{SALMONN-13B}  
&\text{Avg. Y/N (Level-1)}&54.30&42.43&48.07&33.93&48.47&37.32\\
 &\text{Avg. Y/N (Level-2)}&51.84&39.62&47.47&\textbf{34.84}&46.81&33.41\\



\midrule
\multirow{2}{*}{WavLLM-7B}  
&\text{Avg. Y/N (Level-1)}&49.03&34.88&40.40&31.49&41.67&31.67\\
 &\text{Avg. Y/N (Level-2)}&\textbf{51.83}&\textbf{40.72}&\textbf{41.87}&\textbf{33.78}&\textbf{46.81}&\textbf{36.53}\\

\midrule
\multirow{2}{*}{Gemini-1.5-Pro}  
&\text{Avg. Y/N (Level-1)}&56.34&53.82&50.53&49.17&50.27&49.69\\
 &\text{Avg. Y/N (Level-2)}&54.84&47.59&49.60&41.28&\textbf{52.22}&47.55\\


\midrule
\text{GPT-4}  
&\text{Text + Y/N}&93.55&93.52 &98.00&97.99 &91.67&91.65 \\

 
%  & $\triangle$ \\
%  & $\triangle$ \\
\bottomrule
\end{tabular}
}
\caption{Results of Level-2 difficulty analysis with improved prompts across 3 conversational sub-categories (Gender, Age, and Ethnicity Stereotypical Biases). Avg.  denotes the average accuracy and macro-averaged F1 score (\%) of 3 types of Y/N prompts. The \textbf{Bold} is the performance which benefits from Level-2 prompts.}
\label{table:l2-analysis}
% \vspace{-2mm}
\end{table}

==> figure_table/main_chart.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.45]{figure_table/table1.png}
    \caption{Caption}
    \label{fig:main-chart}
\end{figure*}
